A Unified Differentiable Boolean Operator with Fuzzy Logic

This paper presents a unified differentiable boolean operator for implicit solid shape modeling using Constructive Solid Geometry (CSG). Traditional CSG relies on min, max operators to perform boolean operations on implicit shapes. But because these boolean operators are discontinuous and discrete in the choice of operations, this makes optimization over the CSG representation challenging. Drawing inspiration from fuzzy logic, we present a unified boolean operator that outputs a continuous function and is differentiable with respect to operator types. This enables optimization of both the primitives and the boolean operations employed in CSG with continuous optimization techniques, such as gradient descent. We further demonstrate that such a continuous boolean operator allows modeling of both sharp mechanical objects and smooth organic shapes with the same framework. Our proposed boolean operator opens up new possibilities for future research toward fully continuous CSG optimization.

==> sections/figures_only.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=1\linewidth]{figures/vanishing_grad.png}
    \end{center}
    \caption{We demonstrate the importance of avoiding vanishing gradients in an inverse CSG for fitting the union of two circles. 
    %
    Using the traditional \max{}\cite{Godel1932} operator suffers from vanishing gradients, leading to a primitive (left, red) remaining unchanged throughout the optimization and thus failing to reconstruct the target shape. 
    %
    In contrast, our method presented in \refequ{product_fuzzy_logic} avoids vanishing gradient and is able to recover the ground truth (right).}
    \label{fig:vanishing_grad}
\end{figure}

\begin{figure}
    \begin{center}
    \includegraphics[width=1\linewidth]{figures/bilinear_interpolation.png}
    \end{center}
    \caption{Naive bilinear interpolation introduces additional local minima in the occupancy value (top plot) when interpolating between, for instance, \union (top left) and \textsc{difference} (bottom right).}
    \label{fig:bilinear_interpolation}
\end{figure}

\begin{figure}
    \begin{center}
    \includegraphics[width=1\linewidth]{figures/one_shape_overfit.png}
    \end{center}
    \caption{Our method is applicable to different types of primitives, including spheres, planes, quadrics, and tiny neural implicit networks. The choice of primitives will change the inductive bias of the optimization, leading to favoring different results when the amount of primitives is insufficient.}
    \label{fig:one_shape_overfit}
\end{figure}
